Steer Model beyond Assistant: Controlling System Prompt Strength via Contrastive Decoding

Large language models excel at complex instructions yet struggle to deviate from their helpful assistant persona, as post-training instills strong priors that resist conflicting instructions. We introduce system prompt strength, a training-free method that treats prompt adherence as a continuous control. By contrasting logits from target and default system prompts, we isolate and amplify the behavioral signal unique to the target persona by a scalar factor alpha. Across five diverse benchmarks spanning constraint satisfaction, behavioral control, pluralistic alignment, capability modulation, and stylistic control, our method yields substantial improvements: up to +8.5 strict accuracy on IFEval, +45pp refusal rate on OffTopicEval, and +13% steerability on Prompt-Steering. Our approach enables practitioners to modulate system prompt strength, providing dynamic control over model behavior without retraining.

==> table/gsm8k.tex <==
% \begin{table*}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{p{4.2cm}rrrrrrrrr}
% \toprule
% Persona & $\alpha$ & FRE & FK & Exp. FK & $\Delta$FK & Fog & Exp. Fog & $\Delta$Fog & Words\\
% \midrule
%   6-year-old child & 0.0 & -126.95 & 33.26 & 1 & 32.26 & 5.76 & 1 & 4.76 & 323 \\
%    & 1.0 & -204.32 & 43.99 & 1 & 42.99 & 5.57 & 1 & 4.57 & 274 \\
%    & 2.0 & -183.33 & 41.01 & 1 & 40.01 & 5.63 & 1 & 4.63 & 280 \\
%   \addlinespace
%   6-year-old child (detailed) & 0.0 & -144.99 & 35.84 & 1 & 34.84 & 5.13 & 1 & 4.13 & 300 \\
%    & 1.0 & -208.63 & 44.54 & 1 & 43.54 & 4.88 & 1 & 3.88 & 262 \\
%    & 2.0 & -154.14 & 36.86 & 1 & 35.86 & 4.84 & 1 & 3.84 & 284 \\
%   \addlinespace
%   12-year-old child (detailed) & 0.0 & 42.85 & 10.18 & 7 & 3.18 & 7.21 & 7 & 0.21 & 505 \\
%    & 1.0 & -7.36 & 16.87 & 7 & 9.87 & 6.46 & 7 & -0.54 & 428 \\
%    & 2.0 & -14.67 & 17.89 & 7 & 10.89 & 6.49 & 7 & -0.51 & 416 \\
%   \addlinespace
%   12-year-old middle school student & 0.0 & 60.93 & 7.90 & 7 & 0.90 & 9.41 & 7 & 2.41 & 569 \\
%    & 1.0 & 44.27 & 9.93 & 7 & 2.93 & 8.09 & 7 & 1.09 & 535 \\
%    & 2.0 & 37.42 & 10.80 & 7 & 3.80 & 7.85 & 7 & 0.85 & 525 \\
%   \addlinespace
%   18-year-old high school student & 0.0 & 48.93 & 9.85 & 12 & -2.15 & 12.37 & 12 & 0.37 & 568 \\
%    & 1.0 & 51.47 & 9.31 & 12 & -2.69 & 11.17 & 12 & -0.83 & 574 \\
%    & 2.0 & 50.81 & 9.29 & 12 & -2.71 & 10.47 & 12 & -1.53 & 575 \\
%   \addlinespace
%   18-year-old high school student (detailed) & 0.0 & 52.95 & 9.29 & 12 & -2.71 & 11.53 & 12 & -0.47 & 561 \\
%    & 1.0 & 41.97 & 10.60 & 12 & -1.40 & 10.01 & 12 & -1.99 & 539 \\
%    & 2.0 & 40.99 & 10.69 & 12 & -1.31 & 9.95 & 12 & -2.05 & 541 \\
%   \addlinespace
%   25-year-old college graduate & 0.0 & 34.23 & 12.13 & 16 & -3.87 & 15.22 & 16 & -0.78 & 559 \\
%    & 1.0 & 39.08 & 11.38 & 16 & -4.62 & 14.22 & 16 & -1.78 & 577 \\
%    & 2.0 & 41.86 & 10.91 & 16 & -5.09 & 13.71 & 16 & -2.29 & 589 \\
%   \addlinespace
%   25-year-old college graduate (detailed) & 0.0 & 36.46 & 11.91 & 16 & -4.09 & 14.88 & 16 & -1.12 & 559 \\
%    & 1.0 & 37.34 & 11.72 & 16 & -4.28 & 14.05 & 16 & -1.95 & 575 \\
%    & 2.0 & 33.08 & 12.33 & 16 & -3.67 & 14.34 & 16 & -1.66 & 580 \\
%   \addlinespace
% \multicolumn{10}{l}{\emph{Average across all personas (deltas N/A):}}\\
% \addlinespace
%   Average across all personas & 0.0 & 0.55 & 16.29 & -- & -- & 10.19 & -- & -- & 493 \\
%    & 1.0 & -25.77 & 19.79 & -- & -- & 9.31 & -- & -- & 471 \\
%    & 2.0 & -18.50 & 18.72 & -- & -- & 9.16 & -- & -- & 474 \\
% \bottomrule
% \end{tabular}
% \caption{Gemma-3-12B-Instruct essay readability by persona and $\alpha$. Expected grade levels assumed: age 6$\rightarrow$FK/Fog$\approx$1; age 12$\rightarrow$7; age 18$\rightarrow$12; college graduate$\rightarrow$16. Deltas are (observed $-$ expected).}
% \label{tab:gemma_essay_readability}
% \end{table*}

